Cones: Concept Neurons in Diffusion Models for Customized Generation

Human brains respond to semantic features of presented stimuli with different neurons. It is then curious whether modern deep neural networks admit a similar behavior pattern. Specifically, this paper finds a small cluster of neurons in a diffusion model corresponding to a particular subject. We call those neurons the concept neurons. They can be identified by statistics of network gradients to a stimulation connected with the given subject. The concept neurons demonstrate magnetic properties in interpreting and manipulating generation results. Shutting them can directly yield the related subject contextualized in different scenes. Concatenating multiple clusters of concept neurons can vividly generate all related concepts in a single image. A few steps of further fine-tuning can enhance the multi-concept capability, which may be the first to manage to generate up to four different subjects in a single image. For large-scale applications, the concept neurons are environmentally friendly as we only need to store a sparse cluster of int index instead of dense float32 values of the parameters, which reduces storage consumption by 90\% compared with previous subject-driven generation methods. Extensive qualitative and quantitative studies on diverse scenarios show the superiority of our method in interpreting and manipulating diffusion models.

==> section/2.related_work.tex <==
\section{Related Work}\label{sec:related_work}
\subsection{Condition-Guided Synthesis}
Recently, diffusion models \cite{ho2020denoising, dhariwal2021diffusion, rombach2022high} have shone among generative models due to the stability of the training process and the diversity of results, which GANs commonly lack. To further explore its extensibility, a great deal of works have been devoted to diffusion-based conditional generation, which can be broadly classified into two categories. The first one is the approach known as classifier-guidance \cite{liu2023more}, which utilizes a classifier to promote the sampling process of the pre-trained unconditional model. Despite the low cost, the generation effect is not satisfactory. The second one is known as the classifier-free approach \cite{ho2022classifier}, which directly collects a large amount of data pairs for joint optimization under the guarantee of conditional probabilistic derivation. This approach can yield stunningly detailed results but requires great data and training costs. Owing to advances in language \cite{radford2021learning} and cross-modal foundation models \cite{radford2021learning}, much text-to-image work with classifier-free techniques is beginning to emerge, facilitating explicit control on the corresponding semantics and style. However, the expressiveness of text is still limited, and more work wants to utilize additional, conditional information (e.g., reference image, grounding \cite{li2023gligen} and sketch \cite{voynov2022sketch}) to guide the global control further. Relatedly, Cones extends the controllable boundaries of the generated content with customized concepts, focusing mainly on consistency with corresponding reference images.
\subsection{Customized Generation}
Based on the above frozen text-to-image foundation models \cite{saharia2022photorealistic, ramesh2022hierarchical}, some work has exploited the advantages of diffusion models in terms of quality and diversity while editing images locally or globally on different datasets. While most works that require only text (i.e., no region masks) are limited to global editing, some works introduce mask information into the local editing with user-provided masks or text-based localized techniques, showing impressive results. To be more realistic, some works \cite{dreambooth, cosdiff} generate novel renditions of a given subject in new contexts. Furthermore, we explore the concept conflict within the customized generation, breaking the limits of editing a few (i.e., 1 or 2) concepts. 

==> section/teaser.tex <==
\vspace{-0.7cm}
\begin{figure*}[hb]
\centering
\includegraphics[trim={0 0 0 0},clip,width=\textwidth]{fig/fig1.pdf}
\caption{We explore the subject-specific concept neurons in a pre-trained text-to-image diffusion model. Concatenating
multiple clusters of concept neurons representing different persons, objects and background can flexibly generate all related concepts in a single image.} 
\label{fig:teaser} 
\end{figure*}
